Relating Idioms, Arrows and Monads from Monoidal Adjunctions

We revisit once again the connection between three notions of computation: monads, arrows and idioms (also called applicative functors). We employ monoidal categories of finitary functors and profunctors on finite sets as models of these notions of computation, and develop the connections between them through adjunctions. As a result, we obtain a categorical version of Lindley, Yallop and Wadler's characterisation of monads and idioms as arrows satisfying an isomorphism.

==> eptcsdata.tex <==
\providecommand{\firstpage}{18}
\providecommand{\publicationstatus}{R. Atkey and S. Lindley (Eds.): Mathematically\\
Structured Functional Programming (MSFP 2018)\\
EPTCS 275, 2018, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.275.3}{10.4204/EPTCS.275.3}}

